Global Convergence of Adaptive Gradient Methods for An Over-parameterized Neural Network

Adaptive gradient methods like AdaGrad are widely used in optimizing neural networks. Yet, existing convergence guarantees for adaptive gradient methods require either convexity or smoothness, and, in the smooth setting, only guarantee convergence to a stationary point. We propose an adaptive gradient method and show that for two-layer over-parameterized neural networks -- if the width is sufficiently large (polynomially) -- then the proposed method converges \emph{to the global minimum} in polynomial time, and convergence is robust, \emph{ without the need to fine-tune hyper-parameters such as the step-size schedule and with the level of over-parametrization independent of the training error}. Our analysis indicates in particular that over-parametrization is crucial for the harnessing the full potential of adaptive gradient methods in the setting of neural networks.

==> AproofGD.tex <==
Our main observation is the following recursion formula.
\begin{align*}
\norm{\vect{y}-\vect{u}(k+1)}^2 
%&\norm{\vect{y}- \left(\vect{u}(k) + \vI_1 +\vI_2 \right)}^2 \nonumber\\
%\leq &\norm{\vect{y}-\vect{u}(k)}^2 -  2\left(\vect{y}-\vect{u}(k)\right)^\top \left(\vI_1 +\vI_2\right) +2\norm{\vI_1}^2 +2\norm{\vI_2}^2 \nonumber\\
%= &\norm{\vect{y}-\vect{u}(k)}^2 -   2\eta\left(\vect{y}-\vect{u}(k)\right)^\top \left(\mat{H}(k)-\mat{H}(k)^\perp\right) \left(\vect{y}-\vect{u}(k)\right) - 2 \left(\vect{y}-\vect{u}(k)\right)^\top\vect{I}_2 \nonumber \\
%&+2\eta^2\left(\vect{y}-\vect{u}(k)\right)^\top \left(\mat{H}(k)-\mat{H}(k)^\perp\right) ^2 \left(\vect{y}-\vect{u}(k)\right)  + 2\|\vect{I}_2\|^2 \nonumber\\
\approx\norm{\vect{y}-\vect{u}(k)}^2  -   2\eta\left(\vect{y}-\vect{u}(k)\right)^\top\left(I- \eta\mat{H}(k)\right) \mat{H}(k) \left(\vect{y}-\vect{u}(k)\right) \\
%&+  2\eta\left(\vect{y}-\vect{u}(k)\right)^\top\left( \eta\mat{H}^\perp(k) - I \right) \mat{H}^\perp(k) \left(\vect{y}-\vect{u}(k)\right)  +  2\langle{\vect{I}_2- \left(\vect{y}-\vect{u}(k)\right) , \vect{I}_2 \rangle} \nonumber\\
%&+ 2\eta^2\left(\vect{y}-\vect{u}(k)\right)^\top\mat{H}(k)\mat{H}^\perp(k) \left(\vect{y}-\vect{u}(k)\right)
\end{align*}
%where $Term 1$  ensure the decreasing of $\norm{\vect{y}-\vect{u}(k+1)}^2$ and  $\mat{H}^{\perp}$, $\vect{I}_1$, and $\vect{I}_2$ are defined as follows\\
%\begin{itemize}
%\item $
%\mat{H}_{ij}^\perp(k) = \frac{1}{m}\sum_{r \in S_i^\perp}\vect{x}_i^\top \vect{x}_j \indict\left\{\vect{w}_r(k)^\top \vect{x}_i \ge 0, \vect{w}_r(k)^\top \vect{x}_j \ge 0\right\}
%$ is a perturbation matrix.
%\item The entry of the vector $\vect{I}_2$ and  $\vect{I}_1$  accounts for terms that the pattern does change and does not change. That is, for the event
%\[A_{ir} = \left\{\exists \vect{w}: \norm{\vect{w}-\vect{w}_r(0)} \le R, \indict\left\{\vect{x}_i^\top \vect{w}_r(0) \ge 0\right\} \neq \indict\left\{\vect{x}_i^\top \vect{w} \ge 0\right\} \right\} \quad \text{ with } 
%R= \frac{c \lambda_0 \delta}{n^2}\]
%let $S_i = \left\{r \in [m]: \indict\{A_{ir}\}= 0\right\}$, $
%S_i^\perp = [m] \setminus S_i$, and 
%\begin{align*}
%I_1^i &\triangleq  \frac{1}{\sqrt{m}}\sum_{r \in S_i} a_r \left(\relu{\left(
%	\vect{w}_r(k) - \eta\frac{\partial L(\mat{W}(k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_i} - \relu{\vect{w}_r(k)^\top \vect{x}_i}\right) \\
%	I_2^i &\triangleq  \frac{1}{\sqrt{m}}\sum_{r \in S_i^\perp} a_r \left(\relu{\left(
%	\vect{w}_r(k) - \eta\frac{\partial L(\mat{W}(k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_i} - \relu{\vect{w}_r(k)^\top \vect{x}_i}\right) 
%\end{align*}
%
%\end{itemize}
%\simon{@Shirley, Need to define $\vect{I}_1$, $\vect{I}_2$, $\mat{H}^{\perp}$}

==> numeric_adagrad.tex <==
In this section, we use synthetic data to perform numerical experiment to corroborate how the adaptive stepsize robust is  to the choice of the parameters.


\begin{figure}[ht!!!!!]
%\minipage{0.8\textwidth}
\centering
  \includegraphics[width=\linewidth]{figs/iid}
%\endminipage\hfill
\caption{Standard Gaussian i.i.d. with size of training samples $n=500$  and dimension $d=1000$. Hidden layer has nodes $m=600$. $y\in \mathbb{R}^{500}$ is simulated by  standard Gaussian i.i.d.. Observe that $\max_{k} \|\vH(k)\|_2 \leq 1.4$ and $\min_{k} \lambda_{min}\left(\vH(k)\right) \ge 0.4$}
%\end{figure} 
% \begin{figure}[ht!!!!!]
%\minipage{0.8\textwidth}
\centering
  \includegraphics[width=\linewidth]{figs/corr}
%\endminipage\hfill
\caption{Gaussian Correlated (model same as Figure 1).  Observe that $\max_{k} \|\vH(k)\|_2 \leq 63$ and $\min_{k} \lambda_{min}\left(\vH(k)\right) \ge 0.017$ }
\end{figure}

We use synthetic data to illustrate the maximum  and minimum eigenvalues of $\mat{H} (k)$ for each iteration.  Figure 1 uses training dataset with each element follows i.i.d. standard Gaussian, we can see that the largest maximum eigenvalue is around $1.3$ and minimum eigenvalues is around $0.04$ within 100-epoch training. To some extend, it illustrates the cases between  general and best case where each sample are highly uncorrelated.  Figure 2 uses training dataset  follows multivariate Gaussian,we can see that the largest maximum eigenvalue is around $63$ and minimum eigenvalues is around $0.01$ within 100-epoch training.  To some extend, it illustrates the cases between  general and worse case where each sample are highly correlated with no zero mean.
 

